S-BEV: Semantic Birds-Eye View Representation for Weather and Lighting Invariant 3-DoF Localization

We describe a light-weight, weather and lighting invariant, Semantic Bird's Eye View (S-BEV) signature for vision-based vehicle re-localization. A topological map of S-BEV signatures is created during the first traversal of the route, which are used for coarse localization in subsequent route traversal. A fine-grained localizer is then trained to output the global 3-DoF pose of the vehicle using its S-BEV and its coarse localization. We conduct experiments on vKITTI2 virtual dataset and show the potential of the S-BEV to be robust to weather and lighting. We also demonstrate results with 2 vehicles on a 22 km long highway route in the Ford AV dataset.

==> tables/table_b234.tex <==
% Please add the following required packages to your document preamble:
% \usepackage{booktabs}
\begin{table*}
\centering
\caption{Table showing results on the lab dataset}
\label{tab:b234}
\begin{tabular}{@{}cccccccc@{}}
\toprule
&   &          &           &          & \multicolumn{3}{c}{Accuracies}                                                                           \\
Network & RMSE     & log RMSE & Abs. Rel. & Sq. Rel. & $\delta < 1.25$ & $\delta < 1.25^2$ & $\delta < {1.25}^3$ \\ \midrule
Baseline & 0.954806 & 0.344610 & 0.267339 & 0.286913 & 0.586719 & 0.847167 & 0.940082 \\
CVAE & 1.268983 & 0.501691 & 0.518043 & 0.840976 & 0.393357 & 0.665696 & 0.831441 \\ \bottomrule
\end{tabular}
\end{table*}

==> tables/table_corridor.tex <==
% Please add the following required packages to your document preamble:
% \usepackage{booktabs}
\begin{table*}
\centering
\caption{Table showing results on the corridor dataset}
\label{tab:corridor}
\begin{tabular}{@{}cccccccc@{}}
\toprule
&   &          &           &          & \multicolumn{3}{c}{Accuracies}                                                                           \\
Network & RMSE     & log RMSE & Abs. Rel. & Sq. Rel. & $\delta < 1.25$ & $\delta < 1.25^2$ & $\delta < {1.25}^3$ \\ \midrule
Baseline & 0.938408 & 0.215515 & 0.142601 & 0.208943 & 0.857769 & 0.953552 & 0.97917 \\
CVAE & 0.908914 & 0.211417 & 0.140295 & 0.183214 & 0.844014 & 0.956805 & 0.98177 \\ \bottomrule
\end{tabular}
\end{table*}

==> tables/table_living.tex <==
% TODO: fix this, needs to occupy full page width
% Please add the following required packages to your document preamble:
% \usepackage{booktabs}
\begin{table*}
\centering
\caption{Table showing results on the livingroom dataset}
\label{tab:living}
\begin{tabular}{@{}cccccccc@{}}
\toprule
&   &          &           &          & \multicolumn{3}{c}{Accuracies}                                                                           \\
Network & RMSE     & log RMSE & Abs. Rel. & Sq. Rel. & $\delta < 1.25$ & $\delta < 1.25^2$ & $\delta < {1.25}^3$ \\ \midrule
Baseline & 0. & 0. & 0.  & 0. & 0. & 0. & 0.                                \\ 
CVAE & 0.031528 & 0.083085 & 0.039895  & 0.002639 & 0.968042             & 0.994147                                & 0.998906                                \\ \bottomrule
\end{tabular}
\end{table*}


==> tables/table_recon_results_combined.tex <==
% Please add the following required packages to your document preamble:
% \usepackage{booktabs}
\begin{table*}
\centering
\caption{Depth estimation metrics across datasets: Living Room, Lab and Corridor.}
\vspace*{-0.3cm} 
\label{tab:depth}
\begin{tabular}{@{}ccccccccc@{}}
\toprule
 & \multicolumn{1}{l}{} & \multicolumn{4}{c}{Lower is better} & \multicolumn{3}{c}{Higher is better} \\ \cmidrule(lr){3-6} \cmidrule(lr){7-9} 
&   &          & &           &          & \multicolumn{3}{c}{Accuracies}                                                                           \\
Dataset & Mean depth  & RMSE     & log RMSE & Abs. Rel. & Sq. Rel. & $\delta < 1.25$ & $\delta < 1.25^2$ & $\delta < {1.25}^3$ \\ \midrule
\textit{Living room}  & 0.69 & 0.031 &	0.083 &	0.039 &	0.002 &	0.968 &	0.994 &	0.998 \\

% Lab (new) & 0.474137 &	0.176438 &	0.113015 &	0.062705 &	0.88322 &	0.973926 &	0.990921 \\
\textit{Lab [m]} & 1.85 & 0.473 &	0.159 &	0.091 &	0.067 &	0.922 &	0.980 &	0.992 \\
\textit{Corridor [m]} & 4 & 0.908 &	0.211 &	0.140 &	0.183 &	0.844 &	0.956 &	0.980 \\ \bottomrule

\vspace*{-0.8cm} 


\end{tabular}
\end{table*}

==> tables/table_recon_results_comined_no_mean_depth.tex <==
% Please add the following required packages to your document preamble:
% \usepackage{booktabs}
\begin{table*}
\centering
\caption{Depth estimation metrics across datasets: Living Room, Lab and Corridor.}
\vspace*{-0.3cm} 
\label{tab:depth}
\begin{tabular}{@{}ccccccccc@{}}
\toprule
 & \multicolumn{1}{l}{} & \multicolumn{4}{c}{Lower is better} & \multicolumn{3}{c}{Higher is better} \\ \cmidrule(lr){3-6} \cmidrule(lr){7-9} 
&   &          & &           &          & \multicolumn{3}{c}{Accuracies}                                                                           \\
Dataset & RMSE     & log RMSE & Abs. Rel. & Sq. Rel. & $\delta < 1.25$ & $\delta < 1.25^2$ & $\delta < {1.25}^3$ \\ \midrule
\textit{Living room}  &  0.031 &	0.083 &	0.039 &	0.002 &	0.968 &	0.994 &	0.998 \\

% Lab (new) & 0.474137 &	0.176438 &	0.113015 &	0.062705 &	0.88322 &	0.973926 &	0.990921 \\
\textit{Lab [m]} & 0.473 &	0.159 &	0.091 &	0.067 &	0.922 &	0.980 &	0.992 \\
\textit{Corridor [m]} & 0.908 &	0.211 &	0.140 &	0.183 &	0.844 &	0.956 &	0.980 \\ \bottomrule

\vspace*{-0.8cm} 


\end{tabular}
\end{table*}

==> tables/table_topo.tex <==
% Please add the following required packages to your document preamble:
% \usepackage{booktabs}
\begin{table}
\centering
\caption{Topological CNN localization accuracy across datasets}
\vspace*{-0.5cm} 
\label{tab:topotab}
\begin{tabular}{@{}lcc@{}}

\toprule
Dataset              & Accuracy & Off-by-one accuracy \\ \midrule
\textit{Living Room} & 94.35\%      & 100\%                 \\
\textit{Lab}         & 85.77\%  & 99.72\%             \\
\textit{Corridor}    & 97\%     & 100\%               \\ \bottomrule
\vspace*{-0.99cm} 
\end{tabular}
\end{table}

